Online Learning via Offline Greedy Algorithms: Applications in Market Design and Optimization

Motivated by online decision-making in time-varying combinatorial environments, we study the problem of transforming offline algorithms to their online counterparts. We focus on offline combinatorial problems that are amenable to a constant factor approximation using a greedy algorithm that is robust to local errors. For such problems, we provide a general framework that efficiently transforms offline robust greedy algorithms to online ones using Blackwell approachability. We show that the resulting online algorithms have $O(\sqrt{T})$ (approximate) regret under the full information setting. We further introduce a bandit extension of Blackwell approachability that we call Bandit Blackwell approachability. We leverage this notion to transform greedy robust offline algorithms into a $O(T^{2/3})$ (approximate) regret in the bandit setting. Demonstrating the flexibility of our framework, we apply our offline-to-online transformation to several problems at the intersection of revenue management, market design, and online optimization, including product ranking optimization in online platforms, reserve price optimization in auctions, and submodular maximization. We also extend our reduction to greedy-like first order methods used in continuous optimization, such as those used for maximizing continuous strong DR monotone submodular functions subject to convex constraints. We show that our transformation, when applied to these applications, leads to new regret bounds or improves the current known bounds. We complement our theoretical studies by conducting numerical simulations for two of our applications, in both of which we observe that the numerical performance of our transformations outperforms the theoretical guarantees in practical instances.

==> tex/conclusion.tex <==
\section{Conclusion}\label{sec:conclude}
In many settings, decision-makers need to solve NP-hard combinatorial problems
repeatedly over time while the underlying (unknown) reward function changes. Motivated by this,  we study the problem of designing online adversarial algorithms for combinatorial problems that are amenable to a robust greedy approximation algorithm. Using Blackwell strategies, we present a unified framework to transform offline robust greedy approximation algorithms to their online counterparts for both full information and bandit feedback structures. We show that by applying our framework to several applications including maximizing submodular functions, optimizing reserve prices in second price auctions, and optimizing product ranking on online platforms, 
we can obtain improved/new regret bounds.

While we have investigated a selective set of applications of our framework, we believe our framework is general and can capture several other algorithmic problems in revenue management and market design. Examples are online learning in assortment optimization (which is also closely related to submodular optimization and greedy algorithms proved to be useful there as well; cf.~\cite{desir2015capacity,agrawal2019mnl}) and budgeted allocation/Adwords problem in sponsored search auctions (where again greedy algorithms proved to be helpful; cf~\cite{mehta2013online}).  Thus, we believe that investigating  other applications of our framework  is indeed an interesting future research direction.
